Measurement of the ion fraction and mobility of $^{218}$Po produced in $^{222}$Rn decays in liquid argon

We report measurements of the charged daughter fraction of $^{218}$Po as a result of the $^{222}$Rn alpha decay, and the mobility of $^{218}$Po$^+$ ions, using radon-polonium coincidences from the $^{238}$U chain identified in 532 live-days of DarkSide-50 WIMP-search data. The fraction of $^{218}$Po that is charged is found to be 0.37$\pm$0.03 and the mobility of $^{218}$Po$^+$ is (8.6$\pm$0.1)$\times$10$^{-4}$$\frac{\text{cm}^2}{\text{Vs}}$.

==> DS-50-AuthorList-2017-12-12.tex <==
\author[a]{P.~Agnes}
\author[b]{I.~F.~M.~Albuquerque}
\author[c]{T.~Alexander}
\author[d]{A.~K.~Alton}
\author[c]{D.~M.~Asner}
\author[b]{M.~Ave}
\author[c]{H.~O.~Badk}
\author[e]{B.~Baldin}
\author[f,g]{G.~Batignani}
\author[e]{K.~Biery}
\author[h]{V.~Bocci}
\author[i]{G.~Bonfini}
\author[j]{W.~Bonivento}
\author[k,i]{M.~Bossa}
\author[l,m]{B.~Bottino}
\author[n,o]{F.~Budano}
\author[n,o]{S.~Bussino}
\author[p,j]{M.~Cadeddu}
\author[p,j]{M.~Cadoni}
\author[q]{F.~Calaprice}
\author[m]{A.~Caminata}
\author[a,i]{N.~Canci}
\author[i]{A.~Candela}
\author[p,j]{M.~Caravati}
\author[m]{M.~Cariello}
\author[i]{M.~Carlini}
\author[r,s]{M.~Carpinelli}
\author[t,u]{S.~Catalanotti}
\author[t,u]{V.~Cataudella}
\author[v,i]{P.~Cavalcante}
\author[t,u]{S.~Cavuoti}
\author[w]{A.~Chepurnov}
\author[j]{C.~Cical\`o}
\author[u]{A.~G.~Cocco}
\author[t,u]{G.~Covone}
\author[x,y]{D.~D'Angelo}
\author[i]{M.~D'Incecco}
\author[r,s]{D.~D'Urso}
\author[m]{S.~Davini}
\author[t,u]{A.~De~Candia}
\author[h,z]{S.~De~Cecco}
\author[i]{M.~De~Deo}
\author[t,u]{G.~De~Filippis}
\author[t,u]{G.~De~Rosa}
\author[n,o]{M.~De~Vincenzi}
\author[r,s,aa]{P.~Demontis}
\author[ac]{A.~V.~Derbin}
\author[p,j]{A.~Devoto}
\author[ab]{M.~Downing}
\author[q]{F.~Di~Eusanio}
\author[i,y]{G.~Di~Pietro}
\author[h,z]{C.~Dionisi}
\author[ad]{E.~Edkins}
\author[ae]{A.~Fan}
\author[t,u]{G.~Fiorillo}
\author[af]{K.~Fomenko}
\author[ag]{D.~Franco}
\author[i]{F.~Gabriele}
\author[r,s]{A.~Gabrieli}
\author[q,y]{C.~Galbiati}
\author[h,z]{S.~Giagu}
\author[ah]{C.~Giganti}
\author[q]{G.~K.~Giovanetti}
\author[i]{A.~M.~Goretti}
\author[ai]{F.~Granato}
\author[w]{M.~Gromov}
\author[aj]{M.~Guan}
\author[e]{Y.~Guardincerri}
\author[s,ak]{M.~Gulino}
\author[ad]{B.~R.~Hackett}
\author[e]{K.~Herner}
\author[q]{D.~Hughes}
\author[c]{P.~Humble}
\author[a]{E.~V.~Hungerford}
\author[q,i]{An.~Ianni}
\author[n,o]{I.~James}
\author[al]{T.~N.~Johnson}
\author[am]{K.~Keeter}
\author[e]{C.~L.~Kendziora}
\author[q]{G.~Koh}
\author[af]{D.~Korablev}
\author[a,i]{G.~Korga}
\author[an]{A.~Kubankin}
\author[f]{M.~Kuss}
\author[q]{X.~Li}
\author[j]{M.~Lissia}
\author[c]{B.~Loer}
\author[t,u]{G.~Longo}
\author[aj]{Y.~Ma}
\author[an]{A.~A.~Machado}
\author[ap,aq]{I.~N.~Machulin}
\author[k,i]{A.~Mandarano}
\author[n,o]{S.~M.~Mari}
\author[ad]{J.~Maricic}
\author[ai]{C.~J.~Martoff}
\author[h,z]{A.~Messina}
\author[q]{P.~D.~Meyers}
\author[ad]{R.~Milincic}
\author[ab]{A.~Monte}\emailAdd{amonte@fnal.gov}
\author[f]{M.~Morrocchi}
\author[am]{B.~J.~Mount}
\author[ac]{V.~N.~Muratova}
\author[m]{P.~Musico}
\author[ah]{A.~Navrer~Agasson}
\author[ap,aq]{A.~Nozdrina}
\author[an]{A.~Oleinik}
\author[i]{M.~Orsini}
\author[ar,as]{F.~Ortica}
\author[al]{L.~Pagani}
\author[l,m]{M.~Pallavicini}
\author[s]{L.~Pandola}
\author[al]{E.~Pantic}
\author[f,g]{E.~Paoloni}
\author[r,s]{F.~Pazzona}
\author[i]{K.~Pelczar}
\author[ar,as]{N.~Pelliccia}
\author[ab]{A.~Pocar}
\author[e]{S.~Pordes}
\author[q]{H.~Qian}
\author[j]{M.~Razeti}
\author[i]{A.~Razeto}
\author[ad]{B.~Reinhold}
\author[a]{A.~L.~Renshaw}
\author[h]{M.~Rescigno}
\author[ag]{Q.~Riffard}
\author[ar,as]{A.~Romani}
\author[u]{B.~Rossi}
\author[h]{N.~Rossi}
\author[q,i]{D.~Sablone}
\author[af]{O.~Samoylov}
\author[q]{W.~Sands}
\author[n,o]{S.~Sanfilippo}
\author[r,s]{M.~Sant}
\author[k,i]{C.~Savarese}
\author[al]{B.~Schlitzer}
\author[ao]{E.~Segreto}
\author[ac]{D.~A.~Semenov}
\author[af]{A.~Sheshukov}
\author[a]{P.~N.~Singh}
\author[ap,aq]{M.~D.~Skorokhvatov}
\author[af]{O.~Smirnov}
\author[af]{A.~Sotnikov}
\author[q]{C.~Stanford}
\author[r,s,aa]{G.~B.~Suffritti}
\author[t,u,ap]{Y.~Suvorov}
\author[i]{R.~Tartaglia}
\author[m]{G.~Testera}
\author[ag]{A.~Tonazzo}
\author[t,u]{P.~Trinchese}
\author[ac]{E.~V.~Unzhakov}
\author[h,z]{M.~Verducci}
\author[af]{A.~Vishneva}
\author[v]{B.~Vogelaar}
\author[q]{M.~Wada}
\author[d]{T.~J.~Waldrop}
\author[t,u]{S.~Walker}
\author[ae]{H.~Wang}
\author[ae]{Y.~Wang}
\author[ai]{A.~W.~Watson}
\author[q]{S.~Westerdale}
\author[at]{M.~M.~Wojcik}
\author[q]{X.~Xiang}
\author[ae]{X.~Xiao}
\author[aj]{C.~Yang}
\author[a]{Z.~Ye}
\author[q]{C.~Zhu}
\author[at]{G.~Zuzel}

